Mitigating Sovereign Data Exchange Challenges: A Mapping to Apply Privacy- and Authenticity-Enhancing Technologies

Harmful repercussions from sharing sensitive or personal data can hamper institutions' willingness to engage in data exchange. Thus, institutions consider Authenticity Enhancing Technologies (AETs) and Privacy-Enhancing Technologies (PETs) to engage in Sovereign Data Exchange (SDE), i.e., sharing data with third parties without compromising their own or their users' data sovereignty. However, these technologies are often technically complex, which impedes their adoption. To support practitioners select PETs and AETs for SDE use cases and highlight SDE challenges researchers and practitioners should address, this study empirically constructs a challenge-oriented technology mapping. First, we compile challenges of SDE by conducting a systematic literature review and expert interviews. Second, we map PETs and AETs to the SDE challenges and identify which technologies can mitigate which challenges. We validate the mapping through investigator triangulation. Although the most critical challenge concerns data usage and access control, we find that the majority of PETs and AETs focus on data processing issues.

==> 02_Tab1_SlrSearch.tex <==
\caption{Selection Process of the SLR}
\label{tab:slr-search-strategy}
\centering
%\sffamily
\scriptsize
\begin{tabular}{p{0.4em} l cc}
    \toprule
     & & \multicolumn{2}{c}{\textbf{Count}} \\ \cmidrule{3-4}
     \multicolumn{2}{l}{\textbf{Literature Selection Criteria}} & Excluded & Included \\ \midrule
     
     % Iteration 1
     \multicolumn{2}{l}{\textit{Inclusion Criteria}} & & \\
     & Search hits (without temporal restrictions) & 0 & 205 \\
     & Journal and conference hits only & -63 & 142 \\
     & Non-duplicates & -3 & 139 \\ 
     & English publications & -1 & 138 \\ \midrule
     
     % Iteration 2
     \multicolumn{2}{l}{\textit{Exclusion Criteria: Title \& Abstract}} &  & \\
     & Hits with unrelated titles or abstracts & -52 & 86 \\
     & Hits with too broad focus & -2 & 84 \\
     & Hits with unrelated data sovereignty subject & -38 & 46 \\ \midrule
     
     % Iteration 3
     \multicolumn{2}{l}{\textit{Exclusion Criteria: Full-Text}} & & \\
     & Hits focusing on data platforms, storage, or management & -9 & 37 \\
     & Hits without a focus on data exchange/sharing & -16  & 21 \\
     & Hits focusing on legal or governance frameworks & -7 & 14 \\
     \midrule %\midrule
     
     \multicolumn{2}{l}{\textit{\textbf{Total (excl. Backward Search)}}} & \textit{\textbf{-190}} & \textit{\textbf{14}} \\ \midrule
     
     \multicolumn{2}{l}{\textit{Backward Search}} & & \\
     & Search hits & 0 & 42 \\
     & Final hits & -40 & 2 \\ \midrule
     
    \multicolumn{2}{l}{\textbf{Total}} &  & \textbf{16} \\

     
     % Total
     
    \bottomrule
\end{tabular}

